De Sitter space, complexity, and the double-scaled SYK model

The cosmological horizon has an associated entropy suggesting that it might encode a quantum mechanical system on its surface. This has motivated extending the principles of the anti-de Sitter (AdS) space/ conformal field theory (CFT) correspondence to static patch holography. Some of our understanding of the AdS/CFT holography has been catalyzed by exploring the geometric duals to quantum information observables in the CFT side of the correspondence. In particular, holographic complexity captures the evolution of the black hole interior, which is conjectured to be dual to a measure of the difficulty in preparing a quantum circuit on the CFT side. Motivated by these developments, we will propose complexity observables defined in geometric terms for an asymptotically dS spacetime and its putative quantum mechanical dual system. To sharply define complexity observables in the static patch of dS space, they will be anchored to a time-like Dirichlet surface where the dual theory is located, called the stretched horizon. While static patch holography needs much more development in order to reach a level of understanding of the likes of the AdS/CFT correspondence, we hope that the work reported in this thesis allows for crucial steps in this direction.

==> chapters/abstract/abstract.tex <==
% !TeX root = ../../thesis.tex
\chapter{Abstract}                                 \label{ch:abstract}
De Sitter (dS) space is a very interesting playground in theoretical physics of important phenomenological interest. It describes a maximally symmetric space with an accelerated rate of expansion. This is a good approximation for describing our current cosmological era, which also suggests that our universe is evolving asymptotically to become dS space. It is thus relevant to address the questions of a worldline observer in dS space, who only has access to probe a region in spacetime delimited by the cosmological horizon, called the static patch. 

The cosmological horizon has an associated entropy suggesting that it might encode a quantum mechanical system on its surface. This has motivated extending the principles of the anti-de Sitter (AdS) space/ conformal field theory (CFT) correspondence to static patch holography. Some of our understanding of the AdS/CFT holography has been catalyzed by exploring the geometric duals to quantum information observables in the CFT side of the correspondence. In particular, holographic complexity captures the evolution of the black hole interior, which is conjectured to be dual to a measure of the difficulty in preparing a quantum circuit on the CFT side.

Motivated by these developments, we will propose complexity observables defined in geometric terms for an asymptotically dS spacetime and its putative quantum mechanical dual system. To sharply define complexity observables in the static patch of dS space, they will be anchored to a time-like Dirichlet surface where the dual theory is located, called the stretched horizon. While static patch holography needs much more development in order to reach a level of understanding of the likes of the AdS/CFT correspondence, we hope that the work reported in this thesis allows for crucial steps in this direction.

The thesis is divided into four parts.

In part \ref{part:1}, we first provide our motivations for studying static patch holography and define complexity proposals in it. We then review geometric aspects of black holes in asymptotically AdS and dS spacetimes, as well as some basic aspects of holography in both cases. We then present different quantum information-theoretic definitions of complexity in general quantum systems, including the most common use of complexity for states and operators in quantum circuits. Although the exact definition has several ambiguities, it also has some robust properties that only depend on the size of the circuit, including (i) its late time evolution, and (ii) how the circuit reacts under alternating operator insertions, called the switchback effect. These properties are used to define holographic complexity in asymptotically AdS spacetimes.

In part \ref{part:2}, we employ static patch holography to study holographic complexity proposals, originally defined for AdS black holes, to the dS space. We study a general geometry, the extended Schwazschild-dS (SdS) space, which is a multicopy periodic continuation of dS space with (uncharged, non-rotating) black holes. We probe different parts of the background with the complexity observables, which had been previously limited only to the inflating patch of dS space. We also propose a set of holographic complexity observables that resolve a misleading geometric feature found in previous studies, where complexity observables would always diverge at finite time scales with respect to the stretched horizon. Instead, the new proposals display late time growth, and a switchback effect can also be recovered. 

In part \ref{part:3}, we study how to define the complexity in dS space from concrete definitions of complexity in its putative dual microscopic theory. We specialize in a theory that has a pair of double-scaled Sachdev–Ye–Kitaev (DSSYK) models obeying specific constraints, which is presumed to be dual to SdS$_3$ space, and at the same time to a combination of spacelike Liouville CFT$_2$ theories with specific properties (denoted LdS$_2$ CFT). We study the notions of spread complexity, Krylov complexity, query complexity, and a particular proposal for Nielsen complexity in the quantum mechanical and quantum field theory sides of the correspondence, to learn about their geometric description using the currently known entries in the holographic dictionary.

Lastly, in part \ref{part:4} we conclude by summarizing the different lessons from the explorations in the parts above, and how they are connected with each other. We also provide an outlook with questions for future developments.

\instructionsabstract

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}

==> chapters/abstractnl/abstractnl.tex <==
% !TeX root = ../../thesis.tex
\chapter{Beknopte samenvatting}
De Sitter (dS)-ruimte is een zeer interessante speeltuin in de theoretische natuurkunde van groot fenomenologisch belang. Het beschrijft een maximaal symmetrische ruimte met een versnelde uitzetting. Dit is een goede benadering voor het beschrijven van ons huidige kosmologische tijdperk, wat ook suggereert dat ons universum asymptotisch evolueert om dS-ruimte te worden. Het is dus relevant om de vragen te beantwoorden van een wereldlijnwaarnemer in de dS-ruimte, die alleen toegang heeft tot het onderzoeken van een gebied in de ruimtetijd dat wordt begrensd door de kosmologische horizon, de zogenaamde statische patch.

De kosmologische horizon heeft een bijbehorende entropie die suggereert dat deze een kwantummechanisch systeem op het oppervlak zou kunnen coderen. Dit heeft ertoe geleid dat de principes van de anti-de Sitter (AdS) ruimte/conforme veldtheorie (CFT) correspondentie zijn uitgebreid naar statische patchholografie. Een deel van ons begrip van de AdS/CFT-holografie is gekatalyseerd door het onderzoeken van de geometrische dualiteiten naar kwantuminformatie die waarneembaar is in de CFT-kant van de correspondentie. In het bijzonder legt de holografische complexiteit de evolutie van het interieur van het zwarte gat vast, waarvan wordt aangenomen dat deze tweeledig is met een maatstaf voor de complexiteit bij het voorbereiden van een kwantumcircuit aan de CFT-kant.

Gemotiveerd door deze ontwikkelingen zullen we waarneembare complexiteiten voorstellen, gedefinieerd in geometrische termen voor een asymptotisch dS-ruimtetijd en zijn vermeende kwantummechanische duaal systeem. Om de waarneembare complexiteit in het statische deel van de dS-ruimte scherp te definiëren, zullen ze worden verankerd aan een tijdachtig Dirichlet-oppervlak waar de duale theorie zich bevindt, de zogenaamde uitgerekte horizon. Hoewel statische patchholografie nog veel meer ontwikkeling nodig heeft om een niveau van begrip van bijvoorbeeld de AdS/CFT-correspondentie te bereiken, hopen we dat het werk dat in dit proefschrift wordt gerapporteerd cruciale stappen in deze richting mogelijk maakt.

Het proefschrift is verdeeld in vier delen.

In deel \ref{part:1} geven we eerst onze motivaties voor het bestuderen van statische patchholografie en definiëren we daarin complexiteitsvoorstellen. Vervolgens bespreken we de geometrische aspecten van zwarte gaten in asymptotisch AdS- en dS-ruimtetijden, evenals enkele basisaspecten van holografie in beide gevallen. Vervolgens presenteren we verschillende kwantuminformatietheoretische definities van complexiteit in algemene kwantumsystemen, inclusief het meest voorkomende gebruik van complexiteit voor toestanden en operatoren in kwantumcircuits. Hoewel de exacte definitie verschillende dubbelzinnigheden kent, heeft deze ook enkele robuuste eigenschappen die alleen afhankelijk zijn van de grootte van het circuit, waaronder (i) de late evolutie ervan, en (ii) hoe het circuit reageert onder afwisselende operator-invoegingen, het zogenaamde switchback-effect. Deze eigenschappen worden gebruikt om holografische complexiteit in asymptotisch AdS-ruimtetijden te definiëren.

In deel \ref{part:2} gebruiken we statische patchholografie om voorstellen voor holografische complexiteit, oorspronkelijk gedefinieerd voor AdS zwarte gaten, naar de dS-ruimte te bestuderen. We bestuderen een algemene geometrie, de uitgebreide Schwarzschild-dS (SdS)-ruimte, die een periodieke voortzetting van de dS-ruimte met meerdere kopieën is met (ongeladen, niet-roterende) zwarte gaten. We onderzoeken verschillende delen van de achtergrond met de waarneembare complexiteit, die voorheen beperkt was tot de inflatiepatch van dS-ruimte. We stellen ook een reeks waarneembare holografische complexiteitswaarnemingen voor die een misleidend geometrisch kenmerk oplossen dat in eerdere studies werd gevonden, waarbij waarneembare complexiteitswaarnemingen altijd op eindige tijdschalen uiteen zouden lopen met betrekking tot de uitgerekte horizon. In plaats daarvan laten de nieuwe voorstellen een late groei zien, en kan er ook een switchback-effect worden hersteld.

In deel \ref{part:3} bestuderen we hoe we de complexiteit in de dS-ruimte kunnen definiëren op basis van concrete definities van complexiteit in de vermeende dubbele microscopische theorie ervan. Wij leggen ons toe op een theorie die bestaat uit een paar dubbelgeschaalde Sachdev-Ye-Kitaev (DSSYK)-modellen die aan specifieke beperkingen voldoen, waarvan wordt aangenomen dat ze duaal zijn met de SdS$_3$-ruimte, en tegelijkertijd met een combinatie van ruimteachtige Liouville-modellen. CFT$_2$-theorieën met specifieke eigenschappen (aangeduid als LdS$_2$ CFT). We bestuderen de begrippen gespreide complexiteit, Krylov-complexiteit, vraagcomplexiteit en een specifiek voorstel voor Nielsen-complexiteit in de kwantummechanische en kwantumveldtheorie-kanten van de correspondentie, om meer te weten te komen over hun geometrische beschrijving met behulp van de momenteel bekende vermeldingen in het holografische woordenboek.

Ten slotte sluiten we in deel \ref{part:4} af met een samenvatting van de verschillende lessen uit de verkenningen in de bovenstaande delen, en hoe deze met elkaar verbonden zijn. Ook geven we een vooruitblik met vragen voor toekomstige ontwikkelingen.

\instructionsabstract

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/preface/manual/manual.tex <==
% !TeX root = ../../thesis.tex
\chapter{Manual}\label{ch:manual}


\section{Tips and Tricks}

\subsection{Image on the cover page}

If you want to place an image on the cover of the dissertation, you can add
the code underneath to the template (check with your promotor whether this is
allowed).

\paragraph{Include image:}
Search for the \texttt{\textbackslash frontcoverheaderXII} command in
the \texttt{adsphd.cls} file and add the following lines:
\begin{verbatim}
   \begin{textblock*}{56mm}(10mm+#1,15mm)
   \includegraphics[width=56mm,height=20mm]{image/filename}
   \end{textblock*}
\end{verbatim}
Where 56mm is the width, 20mm the height, 10mm the x-location and 15mm the
y-location.

\paragraph{Change cover font color:}
Add the command \texttt{\textbackslash color\{red\}} to the
\texttt{\textbackslash frontcoverheaderXII} command or enclose specific parts.
For example, \texttt{\{\textbackslash color\{red\}\textbackslash
textbf\{\textbackslash @authorf\textbackslash\ \textbackslash @authorl\}}.

\subsection{Full cover page}

\textbf{Important}: most printing services will create their own cover page based
on the details you send them (title, name, affiliation, ...) and do not supply
you with all necessary parameters (e.g., thickness of the paper) because these
differ from machine to machine. Therefore, the generated cover page is only
indicative and probably not used by your printing server (or even correct).


A full cover page (combining front cover, spine and back cover) can be
generated automatically using the command \texttt{make cover} or \texttt{python3 run.py cover}. This creates a pdf
\texttt{\$(COVERPDF);} by default this is \texttt{cover.pdf}.

The width of the spine is set by redefining \texttt{\\adsphdspinewidth} (9mm by default).

It can be seen in the provided \texttt{thesis.tex} that all information necessary to
generate a cover page is contained between two markers

\begin{verbatim}
    %%% COVER: Settings %%%
    ...
    %%% COVER: End settings %%%
\end{verbatim}

DO NOT REMOVE THESE!! They are used by the Makefile!!

The default front and/or back cover page can be overwritten: 

\begin{itemize}
    \item create a file \texttt{mycoverpage.tex}
    \item redefine the commands \texttt{\textbackslash makefrontcovergeneral} and \texttt{\textbackslash makebackcovergeneral}. For
          an example and more information, see the provided file \texttt{mycoverpage.tex}.
\end{itemize}

The cover page in the generated pdf has the following structure:

{\tiny
\begin{verbatim}
    <--rbleed--><--backcoverpage--><--lbleed--><--spine width--><--lbleed--><--frontcoverpage--><--rbleed-->
\end{verbatim}
}

The default bleed (both lbleed and rbleed) is 7mm. I suggest not changing this
value unless you know what you are doing ;) The latter can be done by
redefining \texttt{\textbackslash defaultlbleed} and \texttt{\textbackslash defaultrbleed} respectively.


\subsection{Table of contents}

To remove list of figures, tables and other preface chapters from the table of
contents, search for occurrences of \texttt{\textbackslash addcontentsline} in the file
\texttt{adsphd.cls} and comment them.

\subsection{Small ebook size}

When you add the \texttt{epub} option to the adsphd class the dissertation is
printed to a smaller size to read on a device such as Kindle.

Environments such as tables or tikZ pictures are often sized in absolute values
and not relative to the size of the output. You can wrap them in a resizebox
to enforce scaling:

\begin{verbatim}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{cc}
      ...
    \end{tabular}
  }
\end{verbatim}

\section{Settings for TeXstudio}

If you are working with TeXstudio or other windows latex editors you might want to adjust the editor's settings to allow a proper compilation of the table of contents and list of figures/tables.

\subsection{Custom \textit{makeindex} and \textit{makeglossaries} commands}

According to the \textit{README.md} the tables are indexed through two custom commands. To edit them in TeXstudio open the \textit{Commands} settings (\textit{Options $\to$ Configure TeXstudio...,  Commands} sheet), edit the following fields and press OK.

\textit{Makeindex}:
{\scriptsize
\begin{verbatim}
"C:/Program Files/MiKTeX 2.9/miktex/bin/x64/makeindex.exe" %.nlo -s nomencl.ist -o %.nls
\end{verbatim}}

\textit{Makeglossaries}:
{\scriptsize
\begin{verbatim}
"C:/Program Files/MiKTeX 2.9/miktex/bin/x64/makeindex.exe" %.glo -s %.ist -t %.glg -o %.gls
\end{verbatim}}

Now the customized commands can be launched by using \textit{Tools $\to$ Commands $\to$ MakeIndex/Makeglossaries}. If you want to automatize it in the standard \textit{Build \& View} (F5) and \textit{Compile} (F6) commands look at the following section.

\subsection{Custom Build\&View and Compile meta-commands}

Open \textit{Options $\to$ Configure TeXstudio...,  Build} sheet, edit the following field and press OK.

\textit{Build \& View}:
{\footnotesize\begin{verbatim}
	txs:///pdflatex | txs:///bibtex | txs:///makeglossaries | txs:///makeindex |
	txs:///pdflatex  | txs:///pdflatex
	\end{verbatim}}

To view the PDF once created you have to press F7 (or \textit{Tool $\to$ View}) and the PDF will automatically update in the default viewer whan you modify it. 

If you prefer to directly view the created PDF\textbf{ from the beginning }edit the field as follow:
{\footnotesize\begin{verbatim}
	txs:///pdflatex | txs:///bibtex | txs:///makeglossaries | txs:///makeindex |
	txs:///pdflatex  | txs:///pdflatex | txs:///view-pdf
	\end{verbatim}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage



==> chapters/preface/preface.tex <==
% !TeX root = ../../thesis.tex
\chapter*{Acknowledgements}\label{ch:preface}
To begin with, I would like to thank my supervisor Thomas Van Riet for giving me the opportunity to come to Leuven and, hopefully, start a career as a physicist. His feedback on the thesis has been crucial. To Thomas Hertog for encouraging me to do my first doctoral project on quantum information in dS space, which motivated me to delve into this topic. I thank them both for incorporating me in some of their projects. To Michal Heller and Silke van der Schueren, for collaboration in my first project on holographic complexity in asymptotically dS space, which is the foundation of this whole thesis. To Ahmed Almheiri, Micha Berkooz, Andreas Blommaert, Misha Isachenkov, Thomas Mertens, and Herman Verlinde for inspiring presentations and discussions on the doubled-scaled SYK model and its connection with dS space, which is an important part of the thesis. 

To my collaborators in the PhD (listed in chronological and alphabetic order based on our released works): Kevin Hernandez, Jorge Bernal, Aidan Chatwin-Davies, Thomas Hertog, Natalia Pinzani-Fokeeva, Brandon Robinson, Klaas Parmentier, Thomas Van Riet, Lars Aalsma, Watse Sybesma, Michal P. Heller, Silke Van der Schueren, Rob Tielemans, Jan Pieter van der Schaar, Eyoab Bahiru, Ricardo Espíndola, Ayan K. Patra, Juan F. Pedraza, Edward K. Morvan-Benhaim, Pablo Bueno, Pablo A. Cano, Robie A. Hennigar, Quim Llorens, Filip Landgren, Andrew Rolph, Ben Craps, Juan Hernandez, Mikhail Khramtsov, Maria Knysh, Ashish Shukla, Stefano Baiguera, Nicolò Zenoni, Andrew Svesko, Manus Visser, Rathindra Nath Das, and Upamanyu Moitra. I also thank others with whom I had many useful physics discussions: Matthias Vancraes, Nikolay Bobev, Martin Sasieta, Patrik Nandy, Rotem Berman, Dominik Neuenfeld, and Arvind Shekar. In particular, Lars Aalsma, Stefano Baiguera, Patrik Nandy, Andrew Rolph, and Nicolo Zenoni for answering my questions even after concluding our collaboration, and providing feedback on my work.

I am grateful to the supervisory committee for reading my thesis, for your questions, and suggestions, as well as for sharing some constructive criticism: Nikolay Bobev, Gerda Neyens, Thomas Hertog, Christian Maes, Thomas Van Riet, and the external members: Damián Galante and Michal P. Heller. I also acknowledge the support of the Arenberg Doctoral School during all my time in Leuven. Thanks to Anneleen Marcelis, Filip Sevenants, and the members of the ICTS department: Jo Aerts, Bert Keyaerts, and Greg Vanhove, for your patience in my requests for administrative support or information and technology-related requests; and for managing the ITF in general.

I have to give credit to my office mates for providing advice on several issues, like applying for funding; for postdocs; how to do taxes in Belgium; teaching, and those types of things: Kwinten Frasen, Robert Walker, Axel Molle, Joao Melo and Klaas Parmetier. To everyone in the ITF who had some interesting physics discussions with me at some point: Annelien Vekemans, Xuao Zhang, Sébastien Reymond, Agot Joel Karlsson, Ludovico Machet, Simon Maenaut, Vincent Van Hemelryck, Vasil Dimitrov, Valentin Reys, Juhno Hong, Marina David, Pieter-Jan De Smet, Daniel Mayerson, Igal Arav, Caroline Jonas, Hynek Paul, Caroline Jonas, Flavio Tonioni, Antoine Van Proeyen, Jonathan Menu, Joseph Indekeu, Igal Arav, and, Dionysios Anninos.

Special thanks to the groups I was able to visit during my Ph.D.: the theoretical physics group at Uppsala University, while my supervisor, Thomas Van Riet, was on a sabbatical period; the Delta Institute for Theoretical Physics, where I was hosted mostly by my collaborator Jan Pieter Van der Schaar, and everyone in the string theory group who made the stay more enjoyable. I would also like to thank the members of the HECAP group in the International Centre for Theoretical Physics (ICTP), Trieste in particular: Merhdad Mirbabayi, who hosted me and contributed to many discussions that inspired some of my work; Paolo Creminelli, and Giovanni Villadoro, for helping out in different occasions. I acknowledge the travel contributions from the Delta Institute and the University of Amsterdam, the Research Foundation – Flanders (FWO) (file number K250423N), and the ICTP.

Finally, thanks to my family, my parents Angelica and Jesus, for their patience and support; to my sister Hilda, for her useful advice on different situations; my aunt and uncle Berny and Bruno for hosting me in their house many times; my cousins, nieces, and nephews: Berny Maria, Michael, Emily, Pia, and Bruno Milo for sharing many moments with me. To the landlord Herman, for providing a good place to stay for the majority of my time in Leuven. Finally, to everyone who crossed paths with me in one way or another, thank you.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/publications/publications.tex <==
\chapter*{List of publications}\label{ch:publications}
\begingroup
\def\chapter*#1{}
\begin{thebibliography}{999}
\bibitem{SV}
K.~G.~Hernandez, S.~E.~Aguilar-Gutierrez, J.~Bernal, ``\textit{On the correspondence principle for the Klein-Gordon and Dirac Equations},'' \textbf{Journal of Theoretical and Applied Physics} \textbf{16} (2022), 4
 \href{https://doi: 10.30495/JTAP.162244}{doi: 10.30495/JTAP.162244} [ \href{https://arxiv.org/abs/1907.05842}{arXiv:1907.05842 [quantum-ph]}].

\bibitem{UBCMIT}
S.~E.~Aguilar-Gutierrez, A.~Chatwin-Davies, T.~Hertog, N.~Pinzani-Fokeeva and B.~Robinson, ``\textit{Islands in Multiverse Models},'' \textbf{Journal of High Energy Physics} \textbf{11} (2021), 212
 \href{https://doi:10.1007/JHEP11(2021)212}{doi:10.1007/JHEP11(2021)212} [ \href{https://arxiv.org/abs/2108.01278}{arXiv:2108.01278 [hep-th]}].

\bibitem{Towards}
S.~E.~Aguilar-Gutierrez, K.~Parmentier, T.~Van Riet, ``\textit{Towards an ``AdS  CFT" correspondence from the D$(-1)/$D$7$ system?}," \textbf{Journal of High Energy Physics} \textbf{09} (2022), 249 \href{https://doi.org/10.1007/JHEP09(2022)249}{doi.org/10.1007/JHEP09(2022)249} [ \href{https://arxiv.org/abs/2207.13692}{arXiv:2207.13692 [hep-th]}]

\bibitem{Old}
L.~Aalsma, S.~E.~Aguilar-Gutierrez, and W.~Sybesma, (2022), ``\textit{An Outsider's Perspective on Information Recovery in de Sitter Space}," \textbf{Journal of High Energy Physics} \textbf{01} (2023), 129 \href{https://doi.org/10.1007/JHEP01(2023)129}{doi.org/10.1007/JHEP01(2023)129} [ \href{https://arxiv.org/abs/2210.12176}{arXiv:2210.12176 [hep-th]}].

\bibitem{Gent}
S. E. Aguilar-Gutierrez, M. P. Heller, and S. Van der Schueren, ``\textit{Complexity= Anything Can Grow Forever in de Sitter}," (2023). [Preprint: \href{https://arxiv.org/abs/2305.11280}{arXiv:2305.11280 [hep-th]}].

\bibitem{Adam}
S. E. Aguilar-Gutierrez, T. Hertog, R. Tielemans, J. P. van der Schaar, and T. Van Riet, ``\textit{Axion-de Sitter wormholes}," (2023). \textbf{Journal of High Energy Physics} \textbf{11} (2023), 225 \href{https://doi.org/10.1007/JHEP11(2023)225}{doi.org/10.1007/JHEP11(2023)225} [ \href{https://arxiv.org/abs/2306.13951}{arXiv:2306.13951 [hep-th]}].

\bibitem{China}
S. E. Aguilar-Gutierrez, E. Bahiru, and R. Espindola, ``\textit{The centaur-algebra of observables}," (2023). \textbf{Journal of High Energy Physics} \textbf{03} (2024), 008 \href{https://doi.org/10.1007/JHEP03(2024)008}{doi.org/10.1007/JHEP03(2024)008} [Preprint: \href{https://arxiv.org/abs/2307.04233}{arXiv:2307.04233 [hep-th]}].

\bibitem{Madrid}
S. E. Aguilar-Gutierrez, A. K. Patra, and J. F. Pedraza, ``\textit{Entangled universes in dS wedge holography}," (2023). \textbf{Journal of High Energy Physics} \textbf{10} (2023), 156 \href{https://doi.org/10.1007/JHEP10(2023)156}{doi.org/10.1007/JHEP10(2023)156} [ \href{https://arxiv.org/abs/2308.05666}{arXiv:2308.05666 [hep-th]}].

\bibitem{AdamChina}
S. E. Aguilar-Gutierrez,  R. Espindola, and E. K. Morvan-Benhaim, ``\textit{A teleportation protocol in Schwarzschild-de Sitter space}," (2023) [Preprint: \href{https://arxiv.org/abs/2308.13516}{arXiv:2308.13516 [hep-th]}].

\bibitem{Leuven}
S. E. Aguilar-Gutierrez ``\textit{C=Anything and the switchback effect in Schwarzschild-de Sitter space}," (2023). \textbf{Journal of High Energy Physics} \textbf{03} (2024), 062 \href{https://doi.org/10.1007/JHEP03(2024)062}{doi.org/10.1007/JHEP03(2024)062} [ \href{https://arxiv.org/abs/2309.05848}{arXiv:2309.05848 [hep-th]}].

\bibitem{Barcelona}
S. E. Aguilar-Gutierrez, P. Bueno, P. A. Cano, R. A. Hennigar, Q. Lloren ``\textit{Aspects of higher-curvature gravities with covariant derivatives}," (2023). \textbf{Physical Review D 108 (2023) 12, 124075} \href{https://link.aps.org/doi/10.1103/PhysRevD.108.124075}{10.1103/PhysRevD.108.124075} [Preprint: \href{https://arxiv.org/abs/2310.09333}{arXiv:2310.09333 [hep-th]}].

\bibitem{UK}
S. E. Aguilar-Gutierrez, F. Landgren ``\textit{A multiverse model in dS wedge holography}," (2023). [Preprint: \href{https://arxiv.org/abs/2311.02074}{arXiv:2311.02074 [hep-th]}].

\bibitem{VUBAdam}
S. E. Aguilar-Gutierrez, A. Rolph ``\textit{Krylov complexity is not a measure of distance between states or operators}," (2023). \textbf{Physical Review D 109 (2024) 8, L081701} \href{https://link.aps.org/doi/10.1103/PhysRevD.109.L081701}{10.1103/PhysRevD.109.L081701} [Preprint: \href{https://arxiv.org/abs/2311.04093}{arXiv:2311.04093 [hep-th]}].

\bibitem{Leuven2}
S. E. Aguilar-Gutierrez ``\textit{Entanglement and factorization in axion-de Sitter universes}," (2023). [Preprint: \href{https://arxiv.org/abs/2312.08368}{arXiv:2312.08368 [hep-th]}].

\bibitem{VUBEP}
S. E. Aguilar-Gutierrez, B. Craps, J. Hernandez, M. Khramtsov, M. Knysh, A. Shukla ``\textit{Holographic complexity: braneworld gravity versus the Lloyd bound}," (2023). \textbf{Journal of High Energy Physics} \textbf{03} (2024), 062 \href{https://doi.org/10.1007/JHEP03(2024)173}{doi.org/10.1007/JHEP03(2024)173} [ \href{https://arxiv.org/abs/2312.12349}{arXiv:2312.12349 [hep-th]}].

\bibitem{Leuven3}
S. E. Aguilar-Gutierrez ``\textit{Holographic complexity of axion-de Sitter universes}," (2024). [Preprint: \href{https://arxiv.org/abs/2401.00851}{arXiv:2401.00851 [hep-th]}].

\bibitem{Osaka}
S. E. Aguilar-Gutierrez, S. Baiguera, N. Zenoni ``\textit{Holographic complexity of the extended Schwarzschild-de Sitter space}," (2024). \textbf{Journal of High Energy Physics} \textbf{05} (2024), 201 \href{https://doi.org/10.1007/JHEP05(2024)201}{doi.org/10.1007/JHEP05(2024)201} [ \href{https://arxiv.org/abs/2402.01357}{arXiv:2402.01357 [hep-th]}].

\bibitem{Leuven4}
S. E. Aguilar-Gutierrez ``\textit{Towards complexity in de Sitter space from the double-scaled Sachdev-Ye-Kitaev model}," (2024). [Preprint: \href{https://arxiv.org/abs/2403.13186}{arXiv:2403.13186 [hep-th]}].
\end{thebibliography}
\endgroup

Publications \cite{SV, UBCMIT, Towards, Old, Adam, China, Madrid, AdamChina, Barcelona, UK, VUBAdam, Leuven2, VUBEP, Leuven3} are not discussed in this thesis.

==> mycoverpage.tex <==
% Redefine in this file the commands to generate the front and back cover:
%
%   \makefrontcovergeneral{xskip}{clearpage}
%   \makebackcovergeneral{xskip}{clearpage}
%
% You can start from their definition in adsphd.cls. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own cover page
\makeatletter

%% \renewcommand{\makefrontcovergeneral}[2]{%
%%   %
%%   % Create header
%%   \frontcoverheader{#1}
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Title, subtitle, authorname, text and date can be moved around.
%%   % Change the textblock* commands below. 
%%   %
%%   % Syntax of textblock environment:
%%   % 
%%   %   \begin{textblock*}{width}(xpos,ypos)
%%   %     ...
%%   %   \end{textblock*}
%%   % 
%%   % !! Make sure not to remove the '+#1' part!!!
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Place the title
%%   \begin{textblock*}{120mm}(17.5mm+#1,89.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \raggedright\selectfont\LARGE\sffamily\textbf{\@title}
%%   \end{textblock*}
%%   %
%%   % Place the subtitle
%%   \begin{textblock*}{120mm}(17.5mm+#1,92.0mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily{\@subtitle}
%%   \end{textblock*}
%%   %
%%   % Place the author name
%%   \begin{textblock*}{120mm}(17.5mm+#1,109.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily\@authorf\ \MakeUppercase\@authorl
%%   \end{textblock*}
%%   %
%%   %\begin{textblock}{120}(0,115)
%%   \begin{textblock*}{120mm}(17.5mm+#1,132.0mm)
%%   \textblockcolour{}
%%   \includegraphics*{image/coverfigure}
%%   \end{textblock*}
%%   %
%%   % Place the misc text
%%   \begin{textblock*}{60mm}(96.5mm+#1,187.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   {\small\sffamily Dissertation presented in partial\\
%%   fulfillment of the requirements for\\
%%   the degree of Doctor\\
%%   in \@degree}
%%   \end{textblock*}
%%   %
%%   % Place date
%%   \begin{textblock*}{160mm}(0mm+#1,221.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \begin{center} {\small\sffamily\@date }\end{center}
%%   \end{textblock*}
%%   
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Add footer
%%   \frontcoverfooter{#2}
%% 
%% }

\makeatother

